Learning to Schedule Deadline- and Operator-Sensitive Tasks

The use of semi-autonomous and autonomous robotic assistants to aid in care of the elderly is expected to ease the burden on human caretakers, with small-stage testing already occurring in a variety of countries. Yet, it is likely that these robots will need to request human assistance via teleoperation when domain expertise is needed for a specific task. As deployment of robotic assistants moves to scale, mapping these requests for human aid to the teleoperators themselves will be a difficult online optimization problem. In this paper, we design a system that allocates requests to a limited number of teleoperators, each with different specialities, in an online fashion. We generalize a recent model of online job scheduling with a worst-case competitive-ratio bound to our setting. Next, we design a scalable machine-learning-based teleoperator-aware task scheduling algorithm and show, experimentally, that it performs well when compared to an omniscient optimal scheduling algorithm.

==> code.tex <==

%% probably not necessary. perhaps use a few lines of pseudo-code (again - need help with algorithm/ic/x...)

%"mystyle" code listing set
\lstset{style=mystyle}

	\subsection{Optimal Offline Scheduling - source code}
	\label{mip-code}
	\lstset{language=Python,escapeinside={(*@}{@*)}}         
	\begin{lstlisting}[frame=single,caption=Optimal Offline Scheduler model - Python code for Gurobi Solver] 
	m = self.model
	s = self.scenario
	N = s.num_jobs
	C = s.num_servers
	
	# server dependent job demand (*@ $\frac{j_D}{\eta_{j_\tau}}$ @*)
	demand = []
	for i in range(C):
	demand.append([np.int(np.ceil(job.demand / s.eta[i][job.jtype])) 
	for job in s.jobs])
	
	# server dependent value-density (*@ $j.value * \psi_i$  @*)
	# compatible with previously defined demand
	value_densities = []
	for i in range(C):
	value_densities.append([(job.value * job.psi[i]) / 
	demand[i][j] for j, job in enumerate(s.jobs)])
	
	
	# declare allocation table of binary variable for each 
	# job/time-step/server combination [(i,t,j)]
	ykeys=[(i, t, j) for i in range(C) for t in s.t_range for j in range(N)]
	y = m.addVars(ykeys, vtype=GRB.BINARY, name='y')
	
	# disable allocating jobs before their arrival and after their deadline
	for i in range(C):
	for j in range(N):
	for t in range(s.t_min, s.jobs[j].arrival):
	y[i, t, j].ub = 0
	for t in range(s.jobs[j].deadline + 1, s.t_max + 1):
	y[i, t, j].ub = 0
	
	# demand constraint: job can't be allocated for more than its server-
	# dependent demand more strictly either allocate exactly the demand
	# or not at all 
	alloc = m.addVars(C, N, vtype=GRB.INTEGER, name='alloc')
	completed_f = m.addVars(C, N, vtype=GRB.BINARY, name='completed_f')
	not_allocated_f = m.addVars(C, N, vtype=GRB.BINARY, name='not_allocated_f')
	alloc_f = m.addVars(C, N, vtype=GRB.BINARY, name='alloc_f')
	for i in range(C):
	for j in range(N):
	m.addConstr(alloc[i, j] == y.sum(i, '*', j))
	m.addGenConstrIndicator(completed_f[i, j], True, 
	alloc[i, j] == demand[i][j])
	m.addGenConstrIndicator(not_allocated_f[i, j], True, 
	alloc[i, j] == 0)
	m.addGenConstrOr(alloc_f[i, j], [completed_f[i, j], 
	
	not_allocated_f[i, j]])
	m.addConstr(alloc_f[i, j] == 1)
	
	# capacity constraint - only one job executed at a time
	# on each of the servers
	for t in s.t_range:
	for i in range(C):
	m.addConstr(y.sum(i, t, '*') <= 1)
	
	# affinity constraint - job can only execute on a single server
	# use SOS type 1 constraint
	for j in range(N):
	m.addSOS(type=GRB.SOS_TYPE1, vars=[alloc[i, j] for i in range(C)])
	
	# objective - maximum value_density * allocation
	obj = quicksum([value_densities[i][j] * alloc[i, j] 
	for i in range(C) for j in range(N)])
	m.setObjective(obj, GRB.MAXIMIZE)
	\end{lstlisting}


==> old_feature_table.tex <==
\begin{table}[ht!]
\begin{tabular}{c  p{6cm} } \toprule
Feature & Description \\ \midrule
value & job's value at given server ($v_j$ times $\psi^i_j$) \\
demand & job's total demand at given server ($D_j$ divided by $\eta^i_{j_{\text{type}}}$) \\
rem time & time needed to complete execution \\
to deadline & time left till deadline\\ 
$\psi^i_j$ & job's preference of given server \\
$\eta^i_{j_{\text{type}}}$ & server's efficiency for job's type \\
$\max_i{\psi^i_j}$ & job's highest preference \\
$\max_i{\eta^i_{j_{\text{type}}}}$ & best efficiency for given job type \\
\hline
\text{\# preempted} & number of preempted jobs waiting for given server \\
$\overline{\text{value}}$ & average\\
$\overline{\text{demand}}$ &  of preempted\\
$\overline{\text{rem dur}}$ &  job \\
$\overline{\text{to deadline}}$ & properties\\ 
$\sigma$(\text{demand}) & std. dev\\
$\sigma$(\text{rem dur}) & of preempted\\
$\sigma$(\text{to deadline}) & job \\
$\sigma$(\text{value}) & properties\\
rj demand & running job's \\
rj rem dur & properties\\
rj to deadline & $\ldots$ \\
rj value & $\ldots$ \\ \bottomrule
\end{tabular}
\caption{Job and server features}
\label{tbl:js-features}
\end{table}
